Privacy Guarantees for Cloud-based State Estimation using Partially Homomorphic Encryption

The privacy aspect of state estimation algorithms has been drawing high research attention due to the necessity for a trustworthy private environment in cyber-physical systems. These systems usually engage cloud-computing platforms to aggregate essential information from spatially distributed nodes and produce desired estimates. The exchange of sensitive data among semi-honest parties raises privacy concerns, especially when there are coalitions between parties. We propose two privacy-preserving protocols using Kalman filter and partially homomorphic encryption of the measurements and estimates while exposing the covariances and other model parameters. We prove that the proposed protocols achieve satisfying computational privacy guarantees against various coalitions based on formal cryptographic definitions of indistinguishability. We evaluate the proposed protocols to demonstrate their efficiency using data from a real testbed.

==> Sections/2_related_work.tex <==

\iffalse

\subsection*{Related Work} \label{sec_related_work}


Since R.E. Kalman published his famous paper presenting a recursive solution to the discrete-data linear filtering problem \cite{first_kalman} and its known algorithm was stated \cite{introduction}, the Kalman filter has been the subject of extensive research and applications%, like the area of autonomous or assisted navigation
. These types of applications usually use multiple sensors' measurements \cite{1st_msensor_kalman}. Hence, researchers developed different algorithms for measurement fusion \cite{multi_fuse_meas_colorednoise} \cite{meas_fuse_weights} \cite{multi_fuse_meas_estimates_cov} and estimate fusion \cite{multi_fuse_meas_estimates_cov} \cite{multi_fuse_estimates}. Many researchers are concerned with presenting and analyzing various systems that use distributed Kalman filtering in multi-party estimation algorithms \cite{diffusionKF} \cite{diffKF_cov_intersect} \cite{diffKF_eventTrigger} \cite{diffusionKF_perf}. Because exchanging sensitive information among multiple untrustworthy parties raises privacy concerns, various approaches such as differential privacy \cite{differentialKF} \cite{differentialKF_error}, obfuscation \cite{est_obfuscatePrivacy}, and homomorphic encryption \cite{mparty_privacy_opt_coal} \cite{mparty_privacy_opt} have been proposed to perform computations on sensitive data while keeping the data confidential from untrustworthy parties. 
%Paillier encryption is a type of partially homomorphic encryption (PHE), which is one of the homomorphic cryptography systems that employ asymmetric key schemes. 
This directs the researchers to use partially homomorphic encryption (PHE) in estimation algorithms to preserve date privacy \cite{sets_est_privacy} \cite{privateEst_noKF} \cite{hierEst_privacy_noKF}. 
%Kalman filter algorithms can be used in an encrypted domain to conceal private information while retaining the algorithms' normal effectiveness. 
A secure state estimation using a centralized Kalman filter was proposed \cite{centKF_hybridEnc}, but with the adoption of a hybrid homomorphic encryption scheme. A multi-party dynamic state estimation using the Kalman filter and PHE was proposed in \cite{distrKF_PHE}, and a secure distributed Kalman filter using PHE was proposed in \cite{secure_distrKF}. However, no work has yet provided computational privacy analysis for those estimation algorithms that use the Kalman filter and PHE. Therefore, our contribution in this paper is to investigate the computational privacy of such techniques.  %similar computational privacy analysis was discussed for other systems like the set-based estimation \cite{sets_est_privacy} and cloud-based quadratic optimization \cite{mparty_privacy_opt}.
Considering that other systems have undergone similar computational privacy analyses, such as set-based estimation \cite{sets_est_privacy} and cloud-based quadratic optimization \cite{mparty_privacy_opt}.

\fi

 %\cite{centKF_hybridEnc} %%%*****************all central but hybrid & w/o proof

 %\cite{distrKF_PHE} %%%*****************all distr but w/o proof

 %multiple keys \cite{secure_distrKF}




 
 

%while the computational privacy wasn't previously investigated for the Kalman filter estimation algorithms.

%preserving privacy.
%different approaches to ensure information privacy was appeared like using Homomorphic encryption to process over encrypted data while keeping the data confidential from untrusted parties. 
%and differential privacy \cite{est_obfuscatePrivacy}. Kalman filter differential privacy was discussed in \cite{KF_privacy_utility} \cite{KF_privacy_utility_tracking}  \cite{differentialKF} \cite{differentialKF_error}






\iffalse

%-------------KF----------------------
 kalman paper \cite{first_kalman}

derivations of algorithm and equations \cite{introduction}. 

different approaches for Kalman filter with multiple sensors \cite{1st_msensor_kalman}.

Multi-sensor optimal information fusion Kalman filter: estimates compression (info fusion) \cite{multi_fuse_estimates} 

Multi-Sensor Information Fusion Kalman filter Weighted by Scalars for Systems with Colored Measurement Noises:  \cite{multi_fuse_meas_colorednoise}

Kalman filter based Multiple Sensor Data Fusion in 
systems with time delayed state : KALMAN FILTER BASED MEASUREMENT LEVEL FUSION FOR TIME DELAYED STATE SYSTEMS (MLF) && KALMAN FILTER BASED STATE VECTOR FUSION AND COVARIANCE UNION FUSION FOR TIME DELAYED STATE SYSTEMS (SVF, CUF) \cite{multi_fuse_meas_estimates_cov}

Multi-Sensor Kalman Filtering With Intermittent Measurements
\cite{multi_parallel_intermittent}

A weighted measurement fusion Kalman filter implementation for UAV navigation \cite{meas_fuse_weights}


%%---------------- distr diffusion KF ------------
Diffusion Strategies for Distributed
Kalman Filtering and Smoothing \cite{diffusionKF}

DIFFUSION STRATEGIES FOR DISTRIBUTED KALMAN FILTERING: FORMULATION AND PERFORMANCE ANALYSIS \cite{diffusionKF_perf} 
Event-Triggered Diffusion Kalman Filters: \cite{diffKF_eventTrigger}

Diﬀusion Kalman Filtering Based on Covariance Intersection \cite{diffKF_cov_intersect}

Distributed Kalman Filtering: Consensus, Diffusion, and Mixed \cite{diffKF_cons}


%%----------- distr + diff (no KF) --------------
Distributed Set-Based Observers Using Diffusion Strategy \cite{sets_diff}

%%---------------- mparty comp privacy -----------
privacy preserving set-based estimation using Partially Homomorphic Encryption \cite{sets_est_privacy},

Privacy-Aware Quadratic Optimization Using Partially Homomorphic Encryption: coalitions \cite{mparty_privacy_opt_coal}

Cloud-based Quadratic Optimization with Partially Homomorphic Encryption \cite{mparty_privacy_opt}

%%-------------- state est+privacy --------------
Cooperative State Estimation for Preserving Privacy of User Behaviors in Smart Grid  : obfuscate the privacy-prone data without compromising the performance of state estimation (no encryption) \cite{est_obfuscatePrivacy}

Private State Estimation for Cyber-physical Systems Using
Semi-homomorphic Encryption: (no KF, a secure Luenberger observer ) \cite{privateEst_noKF}

Privacy-Preserving Hierarchical State Estimation in
Untrustworthy Cloud Environments: (No KF) \cite{hierEst_privacy_noKF}

%%----------------KF + privacy -------------------
Privacy-Aware Kalman Filtering: privacy-utility tradeoff / transformation - mapping to another space \cite{KF_transf_privacy}

%@@@ 
Utility and Privacy in Object Tracking from Video Stream using Kalman Filter / privatize by adding noise \cite{KF_privacy_utility_tracking}

Differentially Private Kalman Filtering: assuming centralized trusted server \cite{differentialKF}

Error Bounds and Guidelines for Privacy Calibration in Differentially Private Kalman Filtering \cite{differentialKF_error}


%%---------****** central KF+Enc+privacy -*******-
Secure State Estimation Using Hybrid Homomorphic Encryption Scheme \cite{centKF_hybridEnc} %%%*****************all central but hybrid & w/o proof

%%--**************- KF/distr+Enc+privacy -*******-
Multi-Party Dynamic State Estimation That Preserves Data and Model Privacy: using KF and PHE \cite{distrKF_PHE} %%%*****************all distr but w/o proof

Secure  distributed  Kalman  filter  using  partially homomorphic  encryption : multiple private keys \cite{secure_distrKF}

%%-------- encoding mechanisms-----------------
Localization of cyber-physical systems: privacy, security and efficiency \cite{encoding_localization}


%@@@ 
An encoding mechanism for secrecy of remote state estimation: encoding instead of encryption \cite{encoding_KFest_eavesdropperSafe}


%%---------------- eff. nw use ---------------
%@@@ 
Coalitions for distributed sensor fusion: efficient use of communication bandwidth in a network of distributed sensors. \cite{coalitions_nw_use}




\fi





%In 1960, R.E. Kalman published his famous paper describing a recursive solution to the discrete-data linear filtering problem \cite{r_introduction}. Since that time, due in large part to advances in digital computing, the Kalman filter has been the subject of extensive research and application, particularly in the area of autonomous or assisted navigation.

==> Sections/8_privacy_proof_1.tex <==
 
% In the following Section, we show that the proposed protocols in Section \ref{sec_proposed_solution_1} for privacy-preserving estimation fulfills the privacy goals mentioned in Section \ref{sec_privacy_goals}.

%\section{Privacy Proofs} \label{sec_privacy_proof}

%\vspace{-2mm}
%\begin{proof}
In the next two Sections, we show the privacy features \cite{sets_est_privacy} of the aforementioned protocols \ref{protocol_1} and \ref{protocol_2}.

\section{Privacy of Protocol \ref{protocol_1} for Private Estimation among distributed sensors } \label{sec_privacy_proof_1}

In the following theorem, we outline the privacy characteristics of the protocol against colluding parties of the semi-honest participants: 

\begin{theorem}
\label{th_dist_setup}
Protocol \ref{protocol_1} solves Problem \ref{prob1_stmnt} while preserving computational privacy against
\begin{itemize}
    \item Sensor coalitions.
    \item Cloud coalitions.
    \item Query coalitions if $pm_r>n$, where $p$ the measurement size, $m_r$ is the number of non colluding sensors and $n$ the state size.
\end{itemize}

\end{theorem}
%Proof of theorem \ref{th_dist_setup} is detailed in Section \ref{sec_privacy_proof_1}.

To prove this theorem, 
 we need to show that the coalitions views and simulators are computationally indistinguishable and that the coalition inputs and outputs do not leak extra private information according to Definition \ref{def_semihonest}. The quantities denoted by $\widetilde{()}$ are those obtained by the simulator and they differ from the quantities of the views but follow the same distribution. "Coins" are random numbers used for the encryption process and key generation. $\enc{\Gamma_X}$ for coalition $X$ represents any information that is transferred between other parties over an encrypted channel that may use double encryption with different keys from the homomorphic encryption keys. 
% We consider the following three predefined coalitions in Section \ref{sec_privacy_goals}.
 %We aim to show the privacy features of our protocols \ref{protocol_1} and \ref{protocol_2} against different coalitions in Definitions \ref{def_sensor_caol}, \ref{def_cloud_caol}, and \ref{def_query_caol}
 
 %\subsection{Privacy of Protocol \ref{protocol_1} for Private Estimation among distributed sensors }
 \begin{proof}
 \label{privacy_proof_1}
 In the following proof, We show the privacy features of Protocol \ref{protocol_1} against the following three coalitions:
 \subsection{Coalition of sensors $s$} \label{sec_sensor_coalition}
%The remaining sensor which is not participating in the coalition is denoted by superscript $r$.

If we consider a set of sensors $s=\{s_{1},\dots,s_{t}\}$ participating in the coalition $s$, then $V^{\Pi}_{s}$ represents the coalition view that can be defined as a combination of every sensor view and given by
%The measurement information is considered as input to the sensor and appears as part of the view and the simulator of the coalition. We denote the view of coalition $s$ consisting of the set of sensors $s=\{s_{1},\dots,s_{t}\}$ by $V^{\Pi}_{s}$ which is defined as the combination of every sensor view and given by
\begin{align}
    V^{\Pi}_{s} &= \big(V^{\Pi}_{s_{1}},\dots,V^{\Pi}_{s_{t}} \big)\\
    &= \big( \mathbf{H}_{s,k},\mathbf{y}_{s,k},\mathbf{R}_{s,k}, \enc{\mathbf{y}_{s,k}}, \textit{pk}, \text{coins}_{s}, \enc{\Gamma_s}
    \big), 
    \label{eq_view_sensor_coalition}
\end{align}
%where the subscript $s$ on $H_{s,k},y_{s,k},R_{s,k}$ denotes an array of measurement information of the coalition. 
and the coalition simulator $S_s$ can be obtained by generating 
$\widetilde{\enc{\Gamma_s}}, \widetilde{\enc{y_{s,k}}}$ and $\widetilde{\text{coins}}_{s}$, i.e.
%
\begin{align}
    S_{s} =& \big(\mathbf{H}_{s,k},\mathbf{y}_{s,k},\mathbf{R}_{s,k}, \widetilde{\enc{\mathbf{y}_{s,k}}}, \textit{pk}, \widetilde{\text{coins}}_{s}, \widetilde{\enc{\Gamma_s}}
    \big).
\end{align}
The $\widetilde{\text{coins}}_{s}$ are generated according to the same distribution of $\text{coins}_{s}$ and are independent from other parameters, where the same is true for $\widetilde{\enc{\mathbf{y}_{s,k}}}$ and $\enc{\mathbf{y}_{s,k}}$ as well as $\widetilde{\enc{\Gamma_s}}$ and $\enc{\Gamma_s}$. 
Therefore, we find that $S_{s} \stackrel{c}{\equiv} V^{\Pi}_{s}$.

Furthermore, each measurement information is independent of all others, which makes the coalition unable to infer new information about the measurements of non-colluding sensors. For this coalition, we consider a single step in our proof since the information in each iteration differs from the other iterations. For the next two coalitions, we will prove that each coalition view after $K\in\mathbb{N}^+$ iterations of the protocol is computationally indistinguishable from the view of a simulator that runs the same $K$ iterations.


\subsection{Coalition of sensors $s$ and aggregator}
\label{sec_sensor_aggr_coalition}

Considering $V^{\Pi}_{a}$ is the view of the aggregator, the view of a coalition consisting of a set of sensors  $s=\{s_{1},\dots,s_{t}\}$ and the aggregator can be indicated by $V^{\Pi}_{sa}$ where
\begin{align}
    V^{\Pi}_{sa} =& \big( V^{\Pi}_{s},V^{\Pi}_{a} \big) = \big( V^{\Pi,K}_{s},V^{\Pi,K}_{a} \big),
    \label{eq_view_sensor_aggr_pr1}
\end{align}
 $V^{\Pi,K}_{s}$ and $V^{\Pi,K}_{a}$ are the views of the coalition of sensors and the aggregator respectively after executing $K$ iterations, and %are given by
\begin{align}
%\begin{eqnarray}
\label{eq_add_instant_views}
 V^{\Pi,k+1}_{s}&=( V^{\Pi,k}_{s},I_{s}^{k+1}), \quad \nonumber \\
 V^{\Pi,k+1}_{a}&=( V^{\Pi,k}_{a},I_{a}^{k+1}), \quad k=0, 1,\dots, K-1,
%\end{eqnarray}
\end{align}
where $I_{s}^k$ and $I_{a}^k$ are the new data added at the $k$-th iteration for the sensors coalition $V^{\Pi,0}_{s}=I_{s}^0$ and the aggregator $V^{\Pi,0}_{a}=I_{a}^0$. The view of the aggregator includes the sensors encrypted measurements and the initial estimates from the query node. The measurements at the $k$-th iteration from sensors that are not part of the coalition are marked by subscript $r$ (i.e., $\mathbf{H}_{r,k},\enc{\mathbf{y}_{r,k}},\mathbf{R}_{r,k}$, $k=0, 1,\dots, K-1$). Then, $I_{s}^k$ and $I_{a}^k$ are 
\begin{align}
    I_{s}^k = \big( &\mathbf{H}_{s,k},\mathbf{y}_{s,k},\mathbf{R}_{s,k},\textit{pk},\enc{\mathbf{y}_{s,k}},\text{coins}_{s}, \enc{\Gamma_s}
    \big),
    \label{eq_Instant_view_sensors} \\
    I_{a}^k =\big( &\mathbf{H}_{s,k},\enc{\mathbf{y}_{s,k}},\mathbf{R}_{s,k}, \mathbf{H}_{r,k},\enc{\mathbf{y}_{r,k}},\mathbf{R}_{r,k}, \enc{\hat{\mathbf{x}}_{q,0}}, \nonumber \\ 
    &{\mathbf{P}}_{q,0}, \enc{\hat{\mathbf{x}}_{a,k}}, {\mathbf{P}}_{a,k}, \mathbf{F}, \mathbf{Q_k}, \textit{pk}, \text{coins}_{a} \big), 
    \label{eq_Instant_view_aggr}
\end{align}
%
%The sensors submit their encrypted data to the aggregator, and they do not have any other roles. Hence, a simulator $S_s$ is obtained by generating  $\widetilde{\enc{\Gamma}}$ and $\widetilde{\text{coins}_{s_1}}, dots, \widetilde{\text{coins}_{s_t}}$. 
%
where $\enc{\hat{\mathbf{x}}_{q,0}}, \mathbf{P}_{q,0}$ is the initial estimates from the query node and $\enc{\hat{\mathbf{x}}_{a,k}},\mathbf{P}_{a,k}$ is the $k$ estimates on the aggregator side. %at time step $k$. 
The view of the coalition $V^{\Pi}_{sa}$ is constructed from \eqref{eq_view_sensor_aggr_pr1}-\eqref{eq_Instant_view_sensors}. The simulator of the coalition can be denoted by $S_{sa} =S_{sa}^{K}$, where $S_{sa}^{K}$ is the simulator after executing $K$ iterations. The simulator $S_{sa}$ can be formed using
 \begin{align}
S_{sa}^{k+1}=(S^{k}_{sa},I^{S,k+1}_{sa} ),\quad k=0, 1,\dots, K-1,
 \end{align}
 where $I^{S,k+1}$ is the simulator portion generated at iteration $k+1$, that is given by
\begin{multline}
I^{S,k}_{sa}=\big( \mathbf{H}_{s,k},\widetilde{\enc{\mathbf{y}_{s,k}}},\mathbf{R}_{s,k}, \mathbf{H}_{r,k},\widetilde{\enc{\mathbf{y}_{r,k}}},\mathbf{R}_{r,k}, \widetilde{\enc{\hat{\mathbf{x}}_{q,0}}}, \mathbf{p}_{q,0}, \\ \widetilde{\enc{\hat{\mathbf{x}}_{a,k}}}, \mathbf{P}_{a,k}, \mathbf{F}, \mathbf{Q_k}, \mathbf{y}_{s,k},\textit{pk}, \widetilde{\text{coins}}_{sa},\widetilde{\enc{\Gamma_s}}
\big),
\end{multline}
where its terms are generated or computed as follows:
%% $I^{S,k+1}_{sa}$ is the new data given as follows
% given the inputs and outputs to the coalition $\big(\textit{pk},q, F, Q_k,H_{s,k},R_{s,k},y_{s,k} \big)$, we do the following steps: 
\begin{itemize}
    \item Generate $\widetilde{\enc{\mathbf{y}_{s,k}}}$, $\widetilde{\enc{\mathbf{y}_{r,k}}}$, $\widetilde{\enc{\hat{\mathbf{x}}_{q,0}}}$, $\widetilde{\enc{\hat{\mathbf{x}}_{a,k}}}$ and  $\widetilde{\enc{\Gamma_s}},$ according to the same distribution of $\enc{\mathbf{y}_{s,k}}$, $\enc{\mathbf{y}_{r,k}}$, $\enc{\hat{\mathbf{x}}_{q,0}}$, $\enc{\hat{\mathbf{x}}_{a,k}}$ and $\enc{\Gamma_s}$, respectively.

    \item Compute $\mathbf{P}_{a,k}$ according to \eqref{eqn_enc_kalman3}.
    \item suppose both coins are combined as $\text{coins}_{sa} = (\text{coins}_{a},\text{coins}_{s})$, then generate $\widetilde{\text{coins}}_{sa}$ according to the same distribution.
%    \item Add $H_{r,k}$, $R_{r,k}$, and $\hat{G}_{q,0}$ as they are public information. 
\end{itemize}

%So, based on this generation scheme
Then, all the $\widetilde{\enc{}}$ and $\enc{}$ values are indistinguishable and all other variables in $I^{S,k+1}_{sa}$ are either public or attainable through the protocol steps. Hence, After all iteration steps, we end up with a simulator that achieves $S_{sa} \stackrel{c}{\equiv} V^{\Pi}_{sa}.$
%\begin{align}
% S_{sa} \stackrel{c}{\equiv} V^{\Pi}_{sa}.
%\end{align}
%\begin{align}
%    S_{sa} =& \big(sa, \textit{pk},q, F, Q_k, H_i^{s_1}, y^{s_1}_i, R_i^{s_1},\dots, H_i^{s_t},y^{s_t}_i,R_i^{s_t},\nonumber\\ 
%    & \enc{\hat{c}_{a,k-1}}, \hat{G}_{a,k-1}, \enc{\hat{c}_{a,k}}, \hat{G}_{a,k}, \Lambda_{a,k}, \bar{G}_{a,k}, R_{r,k}, H_{r,k}, \nonumber\\ 
%    & \widetilde{\enc{y_{r,k}}}, \widetilde{\text{coins}}_{sa}, \widetilde{\enc{\bar{c}_{a,k}}} \big).
%\end{align}
%The $(\text{coins}_{a},\text{coins}_{s_1},\dots,\text{coins}_{s_t})$ and $\widetilde{\text{coins}}_{s}$ are generated according to the same distribution and are independent from other parameters. 

Now we need to ensure that the coalition cannot infer any extra private information. The coalition's target is to determine the private measurement of the non-colluding sensors $\mathbf{y}_{r,k}$. The relation between $\enc{\mathbf{y}_{s,k}}$ and $\enc{\mathbf{y}_{r,k}}$ can be derived from \ref{eqn_enc_kalman5} by%and described as
\begin{comment}
\begin{multline}
 \sum\limits_{j\in\mathcal{N}_{r}} \mathbf{K}_{j,k} \enc{\mathbf{y}_{j,k}} = \sum\limits_{j\in\mathcal{N}_{I}} ( \mathbf{K}_{j,k} \mathbf{H}_{j,k} - 1) \enc{\hat{\mathbf{x}}_{a,k-1}} \\
 \oplus \enc{\hat{\mathbf{x}}_{a,k}} \ominus \underbrace{\sum\limits_{j\in\mathcal{N}_{I}-\mathcal{N}{r}} \mathbf{K}_{j,k} \enc{\mathbf{y}_{j,k}}}_{\text{known to the coalition in plaintext}}, \label{eq_unknowns_sensor_aggr_col}
\end{multline}
\end{comment}
\begin{multline}
 \sum\limits_{i\in\mathcal{N}_{r}} \mathbf{K}_{i,k} \enc{\mathbf{y}_{i,k}} = \sum\limits_{i\in\mathcal{N}_{I}} ( \mathbf{K}_{i,k} \mathbf{H}_{i,k} - 1) \enc{\hat{\mathbf{x}}_{a,k-1}} \\
 \oplus \enc{\hat{\mathbf{x}}_{a,k}} \ominus \underbrace{\sum\limits_{i\in\mathcal{N}_{I}-\mathcal{N}{r}} \mathbf{K}_{i,k} \enc{\mathbf{y}_{i,k}}}_{\text{known to the coalition in plaintext}}, \label{eq_unknowns_sensor_aggr_col}
\end{multline}

where $\mathcal{N}_{r}$ is the remaining sensors set, $\mathcal{N}_{I}$ the set of all sensors and $\mathcal{N}_{I}-\mathcal{N}_{r}$ the set participating sensors in coalition. Since the coalition does not have the private key and the query node sends the initial encrypted estimate $\enc{\hat{\mathbf{x}}_{a,0}}$,As a result, we have a system that is undermined in \eqref{eq_unknowns_sensor_aggr_col}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Coalition of sensors $s$ and query node}\label{sec_sensors_query_col}
Let $V^{\Pi}_{q}$ be the view of the query node, then, the view of a coalition consisting of a set of sensors %$s=\{s_{1},\dots,s_{t}\}$ 
and the query is $V^{\Pi}_{sq}$ that defined by

\begin{align}
V^{\Pi}_{sq} =& \big( V^{\Pi}_{s},V^{\Pi}_{q} \big) = \big( V^{\Pi,K}_{s},V^{\Pi,K}_{q} \big),
\end{align}
where 
\begin{align}
\label{eq_add_Instant_views_sensors_query}
V^{\Pi,k+1}_{s}&=( V^{\Pi,k}_{s},I_{s}^{k+1}), \quad \nonumber\\ 
V^{\Pi,k+1}_{q}&=( V^{\Pi,k}_{q},I_{q}^{k+1}),\quad k=0, 1,\dots, K-1,
\end{align}
where $I_{s}^k$ is given in \eqref{eq_Instant_view_sensors}, and $I_{q}^k$ are the new data added from the $k$-th iteration for the query node with $ V^{\Pi,0}_{q}=I_{q}^0$ such that
\begin{align}
\label{eq_Instant_view_Query}
I_{q}^k=\big(\hat{\mathbf{x}}_{q,0},\mathbf{P}_{q,0},\enc{\hat{\mathbf{x}}_{a,k}},\mathbf{P}_{a,k},\hat{\mathbf{x}}_{a,k},\textit{pk},\textit{sk}, \text{coins}_{q}, \enc{\Gamma_{sq}}\big).
\end{align}

The coalition view $V^{\Pi}_{sq}$ can be formed using \eqref{eq_Instant_view_sensors}, \eqref{eq_add_Instant_views_sensors_query} and \eqref{eq_Instant_view_Query}, where the simulator can be constructed like the previous coalition as% The construction of the simulator is similar to Section \ref{sec_sensor_aggr_coalition}. Thus, we focus on the values added in the $k$-th iteration to the simulator. Let the combination of all coins of the parties be denoted by $\text{coins}_{sq} = (\text{coins}_{q},\text{coins}_{s})$. The inputs and outputs to the coalition are ($\textit{pk},\textit{sk},H_{s,k},y_{s,k},R_{s,k},\hat{x}_{a,k},{P}_{a,k},\hat{x}_{q,0},{P}_{q,0}$). Thus, the simulator $S_{sq}^k$ can be easily generated by
\begin{align}
    S_{sq}^k = \big( &\mathbf{H}_{s,k},\mathbf{y}_{s,k},\mathbf{R}_{s,k},\hat{\mathbf{x}}_{q,0},{P}_{q,0},\hat{\mathbf{x}}_{a,k},\mathbf{P}_{a,k},\nonumber \\
    &\widetilde{\enc{\hat{\mathbf{x}}_{a,k}}},\widetilde{\text{coins}}_{sq},\widetilde{\enc{\Gamma_{sq}}}, \textit{pk},\textit{sk}, S_{sq}^{k-1} \big),
\end{align}
where $\left(\widetilde{\enc{\hat{\mathbf{x}}_{a,k}}}, \widetilde{\text{coins}}_{sq}, \widetilde{\enc{\Gamma_{sq}}}\right)$ are generated according to the same distribution of $\left(\enc{\hat{\mathbf{x}}_{a,k}}, \text{coins}_{sq}, \enc{\Gamma_{sq}}\right)$ and are independent from other parameters. Therefore, $S_{sq}^k \stackrel{c}{\equiv} (I_{s}^k,I_{q}^k),$ which proves that 
%\begin{equation}
  $S_{sq} \stackrel{c}{\equiv} V^{\Pi}_{sq}$.
%\end{equation}
To complete our proof, it is important to examine whether the coalition can reveal the private information of the non-colluding $m_r$ sensors. Since the query has the Paillier private key \textit{sk}, we can rewrite \eqref{eq_unknowns_sensor_aggr_col} after decryption
%In case of a coalition between $s$ sensors and the query node, the aim would be to find the measurements of the remaining group, denoted by ${N}_{r}$ with size $m_r$(number of non participating sensors in the coalition). Rewriting \eqref{eq_unknowns_sensor_aggr_col} after decryption -- as the query has the Paillier private key \textit{sk} -- results in
 \begin{align}\label{eq_privacy}
\textbf{K}_{r,k} \textbf{Y}_{r,k}= \mathbf{z}_{s,k},
 \end{align}
where
\begin{comment}
\begin{align}
\label{eq_knowns_sensor_query_col}
&\mathbf{z}_{s,k}=\sum\limits_{j\in\mathcal{N}_{I}} ( \mathbf{K}_{j,k} \mathbf{H}_{j,k}) \hat{\mathbf{x}}_{a,k-1} + \hat{\mathbf{x}}_{a,k} - \sum\limits_{j\in\mathcal{N}_{I} - \mathcal{N}_{r} } \mathbf{K}_{j,k} \; \mathbf{y}_{j,k}, \\
&\textbf{K}_{r,k}=[K_{j_1,k},K_{j_2,k},\dots,K_{{j_{m_r}},k}]\in\mathbb{R}^{n\times pm_r},\nonumber \\
&\textbf{Y}_{r,k}=[y_{j_1,k}^T,y_{j_2,k}^T,\dots,y_{{j_{m_r}},k}^T]^T\in\mathbb{R}^{ pm_r},
\end{align}
\end{comment}
\begin{align}
\label{eq_knowns_sensor_query_col}
&\mathbf{z}_{s,k}=\sum\limits_{i\in\mathcal{N}_{I}} ( \mathbf{K}_{i,k} \mathbf{H}_{i,k}) \hat{\mathbf{x}}_{a,k-1} + \hat{\mathbf{x}}_{a,k} - \sum\limits_{i\in\mathcal{N}_{I} - \mathcal{N}_{r} } \mathbf{K}_{i,k} \; \mathbf{y}_{i,k}, \\
&\textbf{K}_{r,k}=[\mathbf{K}_{i_1,k},\mathbf{K}_{i_2,k},\dots,\mathbf{K}_{{i_{m_r}},k}]\in\mathbb{R}^{n\times pm_r},\nonumber \\
&\textbf{Y}_{r,k}=[\mathbf{y}_{i_1,k}^T,\mathbf{y}_{i_2,k}^T,\dots,\mathbf{y}_{{i_{m_r}},k}^T]^T\in\mathbb{R}^{ pm_r},
\end{align}

where $\mathbf{z}_{s,k}$ is known to the coalition since each $\textbf{K}_{i,k}$ can be calculated using \ref{eqn_enc_kalman4}. We need to examine whether there is no unique retrieval for $Y_{r,k}$ to preserve its privacy, which means that \eqref{eq_privacy} has multiple solutions. %To find the conditions at which the privacy of $Y_{r,k}$ is ensured, we show that there is no unique retrieval for $Y_{r,k}$. This non-unique retrieval requires that \eqref{eq_privacy} has multiple solutions. 
According to \cite[Theorem 6.4]{schott2016matrix}, $\tilde{Y}_{r,k}$ is a solution of \eqref{eq_privacy} for any $X_r \in\mathbb{R}^{pI_r}$ with
 \begin{align}\label{eq_privacy1_1}
\tilde Y_{r,k}=\textbf{K}_{r,k}^{-}\mathbf{z}_{s,k}+(I_{pm_r}-\textbf{K}_{r,k}^{-}\textbf{K}_{r,k})X_r,
 \end{align}
where $\textbf{K}_{r,k}^-$ is any generalized inverse of $\textbf{K}_{r,k}$. 
In order to ensure that \eqref{eq_privacy1_1} has multiple solutions, we need to keep $(I_{pm_r}-\textbf{K}_{r,k}^-\textbf{K}_{r,k})\neq 0$. 
%For every solution $\tilde{Y}_{r,k}$ of \eqref{eq_privacy} there is an $X_r$. For $(I_{pm_r}-\textbf{K}_{r,k}^-\textbf{K}_{r,k})= 0$, the system is consistent and thus has one solution \cite[Theorem 6.1]{schott2016matrix}. Therefore, we aim to find conditions at which $(I_{pm_r}-\textbf{K}_{r,k}^-\textbf{K}_{r,k})\neq 0$ to ensure privacy. 
According to \cite[Theorem 2.8]{schott2016matrix} we have $rank(\textbf{K}_{r,k}^-\textbf{K}_{r,k})\leq \min\{pm_r,n\}$.\\ 
Then, under the condition $pm_r>n$, we have $(I_{pm_r}-\textbf{K}_{r,k}^-\textbf{K}_{r,k})\neq 0$ which preserves the privacy of $Y_{r,k}$.
\end{proof}
%\vspace{-2mm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> Sections/9_privacy_proof_2.tex <==
\section{Privacy of Protocol \ref{protocol_2} for private Estimation among sensor groups }\label{sec_privacy_proof_2}

We summarize the protocol privacy features against colluding parties from semi-honest protocol participants in the following theorem:

\begin{theorem}
\label{th_diff_setup}
Protocol \ref{protocol_2} solves problem \ref{prob2_stmnt} while preserving computational privacy against
\begin{itemize}
    \item Sensor coalitions.
    \item Cloud coalitions.
    \item Query coalitions if $d_r>1$, where $d_r$ is the number of non-colluding groups.
\end{itemize}

\end{theorem}

Following is the theorem-proof similarly to the previous one. 
 
 \begin{proof}
  \label{privacy_proof_2}
In the following proof, we consider the view and simulator for one step (i.e., $k$-th step).% for notational convenience. 
The proof for $K\in\mathbb{N}^+$ steps is the same as previous proof. We prove again the privacy against the following three coalitions:

 \subsection{Coalition of sensors groups $g$}


%The remaining sensor which is not participating in the coalition is denoted by superscript $r$.
Let $V^{\Pi}_{g}$ denote the view of a coalition includes a set of sensor groups $g=\{g_{1},\dots,g_{t}\}$ and defined by
\begin{align}
    V^{\Pi}_{g} = \big(V^{\Pi}_{g_{1}},\dots,V^{\Pi}_{g_{t}} \big) & \\
    = \big( \mathcal{H}_{g,k}, \mathcal{Y}_{g,k}, \mathcal{R} &_{g,k}, \mathbf{P}_{q,k-1}, \hat{\mathbf{x}}_{q,k-1}, \mathbf{P}^{-}_{g,k}, \nonumber \\
    \hat{\mathbf{x}} &^{-}_{g,k}, \textit{pk}, \enc{\hat{\mathbf{x}}^{-}_{g,k}}, coins_g, \enc{\Gamma_g}
    \big),
\end{align}
where the subscript $g$ denotes items owned by the coalition. Each sensor group submit only its encrypted prior estimate to the aggregator. Hence, the simulator $S_g$ is defined by
\begin{multline}
        S_{g} = \big( \mathcal{H}_{g,k}, \mathcal{Y}_{g,k}, \mathcal{R}_{g,k}, \mathbf{P}_{q,k-1}, \hat{\mathbf{x}}_{q,k-1}, \mathbf{P}^{-}_{g,k}, \\
        \hat{\mathbf{x}}^{-}_{g,k}, \textit{pk}, \widetilde{\enc{\hat{\mathbf{x}}^{-}_{g,k}}}, \widetilde{coin}_g, \widetilde{\enc{\Gamma_g}} \big),
\end{multline}
and $\widetilde{\enc{\hat{\mathbf{x}}^{-}_{g,k}}}$,  $\widetilde{\text{coins}}_{g}$ and $\widetilde{\enc{\Gamma_g}}$ are generated with the same distribution of $\enc{\hat{\mathbf{x}}^{-}_{g,k}}, coins_g, \enc{\Gamma_g}$ and are independent from other parameters. Therefore, we find that $ S_{g} \stackrel{c}{\equiv} V^{\Pi}_{g}$. Also, the coalition cannot infer any further information about other estimates of the non-colluding groups.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Coalition of sensor groups $g$ and the aggregator} 

The coalition view is defined by
\begin{align}
    V^{\Pi}_{ga} =& \big( V^{\Pi}_{g},V^{\Pi}_{a}  \big)
\end{align}
where
\begin{multline}
    V^{\Pi}_{a} = \big(\enc{\hat{\mathbf{x}}^{-}_{g,k}}, \mathbf{P}^{-}_{g,k}, \enc{\hat{\mathbf{x}}^{-}_{r,k}}, \mathbf{P}^{-}_{r,k},\enc{\hat{\mathbf{x}}_{a,k}}, \mathbf{P}_{a,k}, \mathbf{F},
    \\ \mathbf{Q_k}, \text{coins}_a, \textit{pk} \big).
\end{multline}
%where $\enc{\hat{x}^{-}_{r,k}}$ and $\hat{P}_{r,k}$ represents the encrypted estimate and the covariance of the remaining sensor groups which are not part of the coalition. 
The simulator $S_{ga}$ can be constructed by calculating $\mathbf{P}^{-}_{g,k}$ and $\mathbf{P}^{-}_{r,k}$ using \eqref{eqn_sensor_gp_cov}, $\mathbf{P}^{-}_{a,k}$ using \eqref{eqn_sensor_gp_agg_cov}, and generating $\widetilde{\enc{\hat{\mathbf{x}}^{-}_{g,k}}}, \widetilde{\enc{\hat{\mathbf{x}}^{-}_{r,k}}}, \widetilde{\enc{\hat{\mathbf{x}}_{a,k}}}$, and $\widetilde{\enc{\Gamma_g}}$ as before.
%from the input and output ($\mathcal{H}_{g,k}, \mathcal{R}_{g,k}, \mathcal{Y}_{g,k}, \textit{pk},  F, G, w_k, Q_k$). Specifically:
\begin{comment}
\begin{itemize}
    %\item Add $\mathcal{H}_{r,k}$ and $\mathcal{R}_{r,k}$ as they are public information. 
    \item Calculate $P^{-}_{g,k}$ and $P^{-}_{r,k}$ using \eqref{eqn_sensor_gp_cov}.
    \item Calculate ${P}^{-}_{a,k}$ using \eqref{eqn_sensor_gp_agg_cov}.
    \item Generate $\widetilde{\enc{\hat{x}^{-}_{g,k}}}, \widetilde{\enc{\hat{x}^{-}_{r,k}}}, \widetilde{\enc{\Gamma_g}}$, and $\widetilde{\enc{\hat{x}_{a,k}}}$ according to the distributions of the original values. 
    \item Let the combination of coins of all parties be $\text{coins}_{ga} = (\text{coins}_{a},\text{coins}_{g})$. Generate $\widetilde{\text{coins}}_{ga}$ according to the distribution of $\text{coins}_{ga}$.
    \item Compute $\hat{x}^{-}_{g,k}$ according to \eqref{eqn_sensor_gp_estimate}.
\end{itemize}
\end{comment}
%We end up with the simulator
\begin{multline}
    S_{ga} = \big(\mathcal{H}_{r,k}, \mathcal{R}_{r,k}, \mathcal{H}_{g,k}, \mathcal{Y}_{g,k}, \mathcal{R}_{g,k},\mathbf{P}_{q,k-1}, \hat{\mathbf{x}}_{q,k-1},\\
    \mathbf{P}^{-}_{g,k}, \hat{\mathbf{x}}^{-}_{g,k}, {P}^{-}_{r,k}, \widetilde{\enc{\hat{\mathbf{x}}^{-}_{r,k}}}, \widetilde{\enc{\hat{\mathbf{x}}^{-}_{g,k}}},\widetilde{\enc{\hat{\mathbf{x}}_{a,k}}}, \mathbf{P}_{a,k},\\
     F, Q_k, \textit{pk}, \widetilde{\text{coins}}_{ga}, \widetilde{\enc{\Gamma_g}} \big).
\end{multline}

Thus, we find that $ S_{ga} \stackrel{c}{\equiv} V^{\Pi}_{ga}$. To ensure that the coalition cannot find the remaining groups estimates, we use \eqref{eqn_sensor_gp_agg_estimate} to describe the relation between group estimates as
 %The target of this coalition is to get the state estimates of the remaining groups, denoted by ${N}_{r}$ with size $d_r$. The estimates of the groups are related by
 \begin{align}
 \sum\limits_{j\in\mathcal{N}_{r}}{(\mathbf{P}^{-}_{g_{j},k})^{-1} \enc{\hat{\mathbf{x}}^{-}_{g_{j},k}}} = &(\mathbf{P}^{-}_{a,k})^{-1} \enc{\hat{\mathbf{x}}^{-}_{a,k}} \nonumber
 \\ &\ominus \underbrace{\sum\limits_{j\in\mathcal{N}/r} {(\mathbf{P}^{-}_{g_{j},k})^{-1} \enc{\hat{\mathbf{x}}^{-}_{g_{j},k}}}}_{\text{known to the coalition in plaintext}}, \label{eq_unknowns_sensorgps_aggr_col}
\end{align}

where ${N}_{r}$ is the set of non-colluding groups with size $d_r$. %The right hand side of \eqref{eq_unknowns_sensorgps_aggr_col} is known to the coalition. 
Since the coalition does not have the private key, the privacy of the remaining groups estimates can be guaranteed.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Coalition of sensor groups $g$ and the query node}


The coalition view $V^{\Pi}_{gq}$ is defined as $V^{\Pi}_{gq} = \big( V^{\Pi}_{g},V^{\Pi}_{q} \big)$ where %$V^{\Pi}_{q}$ given by
\begin{align}
    V^{\Pi}_{q} =& \big( \enc{\hat{\mathbf{x}}_{a,k}},\hat{x}_{a,k}, \mathbf{P}_{a,k}, 
 \textit{pk},\textit{sk}, \text{coins}_q, \enc{\Gamma_q} \big).
\end{align}

And the simulator $S_{gq}$ can be constructed as before 
\begin{multline}
S_{gq} = \big(\mathcal{H}_{g,k}, \mathcal{Y}_{g,k}, \mathcal{R}_{g,k}, \mathbf{P}^{-}_{g,k}, \hat{\mathbf{x}}^{-}_{g,k},
\\  \widetilde{\enc{\hat{\mathbf{x}}_{a,k}}},\hat{\mathbf{x}}_{a,k}, \mathbf{P}_{a,k}, \textit{pk}, \textit{sk}, \widetilde{\text{coins}}_{gq}, \widetilde{\enc{\Gamma_q}} \big).
\end{multline}
thus we conclude that $S_{gq} \stackrel{c}{\equiv} V^{\Pi}_{gq}$. To investigate the privacy of the non-colluding groups' estimates, we use \eqref{eq_unknowns_sensorgps_aggr_col} after decryption as the query has the private key \textit{sk}.
%The target of this coalition is to get the estimates of the remaining groups, denoted as before by $\mathcal{N}_{r}$ with size $d_r$. Rewriting \eqref{eq_unknowns_sensorgps_aggr_col} after decryption -- as the query has the Paillier private key \textit{sk} -- results in
 \begin{align}\label{eq_privacy_protocol_2}
\textbf{P}_{r,k} \textbf{X}_{r,k}= \mathbf{z}_{g,k},
 \end{align}
with
\begin{align}
\mathbf{z}_{g,k}&=(\mathbf{P}^{-}_{a,k})^{-1} \hat{\mathbf{x}}^{-}_{a,k} - 
    \sum\limits_{j\in\mathcal{N}/r} {(\mathbf{P}^{-}_{g_{j},k})^{-1} \hat{\mathbf{x}}^{-}_{g_{j},k}}, \\
%\textbf{P}_{r,k} &=[P_{g,k}^{j_1}I_n,P_{g,k}^{j_2}I_n,\dots,P_{g,k}^{j_{d_r}}I_n]\in\mathbb{R}^{n\times nd_r},\\
\textbf{P}_{r,k} &=[\mathbf{P}_{g,k}^{j_1}, \mathbf{P}_{g,k}^{j_2},\dots,\mathbf{P}_{g,k}^{j_{d_r}}]\in\mathbb{R}^{n\times nd_r},\\
\textbf{X}_{r,k}&=[\mathbf{x}_{j_1,k}^T, \mathbf{x}_{j_2,k}^T,\dots,\mathbf{x}_{j_{d_r},k}^T]^T\in\mathbb{R}^{ nd_r},
\end{align}
where $z_{g,k}$ is known to the coalition as $\hat{\mathbf{x}}^{-}_{a,k}$ and $\mathbf{P}^{-}_{a,k}$ can be calculated using \eqref{eq_diff_est_tUpdt} and \eqref{eq_diff_cov_tUpdt} assuming that $\mathbf{F}$ and $\mathbf{Q}_{k}$ are public and $\mathbf{F}$ is invertible. If $\mathbf{F}$ isn't invertible, the privacy of remaining will be guaranteed against all coalitions.
Similarly to proof \ref{privacy_proof_1} and according to \cite[Theorem 6.4]{schott2016matrix}, $\tilde{X}_{r,k}$ is a solution of \eqref{eq_privacy_protocol_2} for any $X_r \in\mathbb{R}^{nd_r}$ where
 \begin{align}\label{eq_privacy2}
\tilde X_{r,k}=\textbf{P}_{r,k}^{-1} z_{g,k} + (I_{nd_r}-\textbf{P}_{r,k}^{-1} \textbf{P}_{r,k} ) X_r,
 \end{align}
with $\textbf{P}_{r,k}^{-1} $ is any generalized inverse of $\textbf{P}_{r,k}$.% For every solution $\tilde{X}_{r,k}$ of \eqref{eq_privacy_protocol_2} there is a $X_r$. If $I_{nd_r}-\textbf{P}_{r,k}^{-1} \textbf{P}_{r,k} = 0$, we end up with a consistent system with one solution \cite[Theorem 6.1]{schott2016matrix}. Thus, 
We aim to find conditions at which $I_{nd_r}-\textbf{P}_{r,k}^{-1} \textbf{P}_{r,k} \neq 0$ to ensure privacy. We have $rank(\textbf{P}_{r,k}^{-1} \textbf{P}_{r,k} )\leq \min\{nd_r,n\}$ according to \cite[Theorem 2.8]{schott2016matrix}. Thus, under the condition $d_r>1$, the privacy of $X_{r,k}$ is guaranteed.
%it follows that $I_{nd_r}-\textbf{P}_{r,k}^{-1} \textbf{P}_{r,k} \neq 0$ which ensures privacy of $X_{r,k}$.

\end{proof}
